The Calculus of Blowups on a Ruled Surface

The purposes of this article are threefold. First, to determine numerically when an arbitrary blowup of a smooth surface is smooth. We show the surface is smooth if and only if certain rational parameters involving log discrepancy and multiplicity of the exceptional divisors form a generalised Farey sequence within the dual graph of divisors. Second, in doing the above we provide an exposition of the Berkovich projective line $\mathbb P^1_{\text{an}}(\mathbb K)$ over the Puiseux series as a universal dual graph for divisors on a ruled surface. Third, to explain how non-Archimedean skew products interact with this multiplicity structure of the tree.

==> pictures/tikzpreamble.tex <==
% total axis width key: sets x so the whole axis fits the requested width
\newif\ifshowinfty
\newif\ifshowplusinfty
\newif\ifshowminusinfty

\makeatletter
\tikzset{
  axis width/.code={
    \pgfmathsetmacro{\Span}{\RightVal-\LeftVal}
%    \pgfmathsetmacro{\Span}{\RightInt-\LeftInt}
    \pgfmathsetmacro{\InfPad}{\InfPadFactor*\Span}
    \pgfmathsetmacro{\TotalSpan}{\Span}
     \ifshowminusinfty
      \pgfmathsetmacro{\TotalSpan}{\Span + \InfPad}
    \fi
     \ifshowplusinfty
      \pgfmathsetmacro{\TotalSpan}{\Span + \InfPad}
    \fi
    \ifshowinfty
      \pgfmathsetmacro{\TotalSpan}{\Span + 2*\InfPad}
    \fi
    % parse requested width (#1) as a TeX length into a dimen register
    \pgf@x=#1\relax

    % compute x-unit in pt:  (width in pt)/(TotalSpan)
    \pgfmathsetmacro{\Xunitpt}{\strip@pt\pgf@x/\TotalSpan}
    \tikzset{x=\Xunitpt pt}

    % handy infinity x-positions
    \pgfmathsetmacro{\xLinf}{\LeftVal-\InfPad}
    \pgfmathsetmacro{\xRinf}{\RightVal+\InfPad}
%    \pgfmathsetmacro{\xLinf}{\LeftInt-\InfPad}
%    \pgfmathsetmacro{\xRinf}{\RightInt+\InfPad}
  }
}
\makeatother

